Impact of Acceleration/deceleration Limits on the String Stability of Adaptive Cruise Control

This paper demonstrates that the acceleration/deceleration limits in ACC systems can make a string stable ACC amplify the speed perturbation in natural driving. It is shown that the constrained acceleration/deceleration of the following ACCs are likely to cause speed overshoot to compensate for an extra large/small spacing. Additionally, we find that the constrained deceleration limits can also jeopardize safety, as the limited braking power produces extra small spacing or even crashes. The findings are validated through experiments on real cars. The paper suggests that the ACC parameter space should be extended to include the acceleration/deceleration limits considering their significant role exposed here. Through numerical simulations of ACC platoons, we show i) a marginal string stable ACC is preferable due to the smaller total queue length and the shorter duration in congestion; ii) congestion waves in a mixed ACC platoon largely depend on the sequence of vehicles provided different acceleration/deceleration limits, and iii) the safety hazard caused by the constrained deceleration limits is more significant in mixed ACC platoons when string unstable ACCs exist.

==> recycle.tex <==
% With a constant time headway, the simplest CF model only reacts to distance change from a desired spacing:
% \begin{align}
%     a &= k_v (s-\eta- v \tau) = -\tau k_v \cdot v + k_v\cdot s  -\eta k_v\\
%     \ddot{x_n} &= f_{v} (v-v_{eq}) +f_{\Delta x} (\Delta x_n - \Delta x_{n,eq}) \label{simple-liear-CF} 
% \end{align}

% Similarly, in this case we have $f_v = -\tau k_v$, $f_{\Delta v}=0$ and $f_{\Delta x} = k_v$. The SS condition in \eqref{SS-cond-CF} reduces to:

% \begin{align}
%     \tau^2 k_v^2 -2 k_v & \ge 0 \nonumber \\
%     \tau^2 k_v-2 & \ge 0 
% \end{align}

% While the above model might be the simplest linear planner, we found in factory ACC algorithm \citep{}, the lead vehicle speed $v_l$ is used to replace the ego vehicle speed $v$. 

% To fix this, \eqref{CF-approx} needs to be extended as:

% \begin{align}
%     \Ddot{x_n} \approx \ddot{x_{n,eq}} + f_{n,v} (\dot{x_n}-\dot{x_{n,eq}}) + f_{n,\Delta x}(\Delta x_n - \Delta x_{n,eq}) + f_{n,\Delta v}(\Delta \dot{x_n}-\Delta \dot{x_{n,eq}}) + \ddot{x_{n-1,eq}}
%      \label{CF-approx-extend}
% \end{align}

% Notice that \eqref{linear-vlead-CF} does not require the proximity of the equilibrium point, because such dynamics always hold. However, \eqref{simple-liear-CF} is equivalent to \eqref{linear-vlead-CF} around equilibrium point considering that $\ddot{x_{n-1}}=0$ and $v_l = v$. Such equivalence indicate for the $l_2$ stability condition, those two linear models do not vary from each other.

% We argue that it is not fair to say such two linear models have the same SS, in the next section we will show the different SS of the two linear CF models using simulations below.



% Let $y_n$ and $u_n$ denote the headway and speed variation from equilibrium state.
% \begin{align}
%     \dot{y_n} &= \dot{x_{n-1}} - \dot{x_n} = u_{n-1} - u_n\\
%     \dot{u_n} &= \dot{v_n} =      \begin{cases}
%       k_v y_n + (1-k_v H) \dot{u_{n-1}} &\quad\text{near equilibrium when unconstrained}\\
%       a_{max}/v_{max}(v_{max}- v_{n,eq} - u_n) &\quad\text{if constrained}
%      \end{cases}
% \end{align}

% Take the Laplace transform and let $U(s) = \mathcal{L}\{u(t)\}$, and $Y(s) = \mathcal{L}\{y(t)\}$.
% \begin{align}
%     Y(s) &= \mathcal{L}\{ \int (u_{n-1}-u_n) dt \} = \frac{1}{s} [\mathcal{L}\{ u_{n-1}(t)\} -\mathcal{L}\{ u_n(t) \}]= \frac{1}{s} [U_{n-1}(s) - U_n(s)]   \label{Y(s)}   \\
%     sU_n(s) &= \begin{cases}
%       k_v Y(s) +(1-k_v H) \cdot s U_{n-1}(s) &\quad\text{near equilibrium}\\
%       a_{max}/v_{max}(v_{max}- v_{n,eq}- u_n) &\quad\text{when acceleration is constrained}
%      \end{cases}
%      \label{Un(s)-acceleration}
% \end{align}

% Substitute \eqref{Y(s)} into \eqref{Un(s)-acceleration}, we have the transfer function:
% \begin{align}
%     sU_n(s) &=  \begin{cases}
%       k_v/s [U_{n-1}(s) - U_n(s)] + (1-k_v H) s U_{n-1}(s) &\quad\text{if unconstrained}\\
%      a_{max} (v_{max}- v_{n,eq})/(sv_{max}) - U(s) &\quad\text{if constrained}
%      \end{cases} 
% %   \Gamma(s) &= \frac{U_{n}(s)}{U_{n-1}(s)} = \frac{(1-k_v H)s^2+k_v}{s^2+k_v}
% \end{align}

% Notice that if the follower $n$ is constrained by its acceleration limits, there is no transfer function any more. One can derive the $U_n(s)$ explicitly:

% \begin{equation}
%     U_n(s) = \frac{a_{max}(v_{max}-v_{n,eq})}{v_{max}(s+1)s}
% \end{equation}

% Assuming the lead vehicle has a large acceleration $a_l$, we can also derive the lead vehicle speed profile in Laplace transform $U_{n-1}(s)$:

% \begin{equation}
%     U_{n-1}(s) = \frac{a_l}{s}
% \end{equation}

% Thus the speed to speed transfer function is:

% \begin{equation}
%     \Gamma(s) &= \frac{U_{n}(s)}{U_{n-1}(s)} = \frac{a_{max}(v_{max}-v_{n,eq})}{a_l v_{max}} \frac{1}{(s+1)}
% \end{equation}

% where we need $|1-k_vH|<1$ to guarantee the SS. Notice that $k_v>0$ and vary at different speed levels. Time headway is usually a constant with short, medium and far options. Thus the SS condition reduces to:
% \begin{equation}
%     k_v (v) < 2/H
%     \label{SS-condition}
% \end{equation}




% The conflict between comfortableness and speed dampening.


% \textbf{Another proof approach:}

% \begin{proof} We first convert the time-domain planner trajectory in \eqref{factory-ACC-vlead} into frequency domain:
% \begin{equation}
%     v_{n}(j\omega) = k_v [x_{n-1}(j\omega) - x_{n}(j\omega) - H v_{n-1}(j\omega) - s_j] + v_{n-1}(j\omega)
%     \label{linear_freq}
% \end{equation}
% Substitute position variables using $x_{n-1}(j\omega) = v_{n-1}(j\omega)/j\omega$, and $x_{n}(j\omega) = v_{n}(j\omega)/j\omega$, we can derive the acceleration to acceleration transfer function similar to \eqref{transfer-function} for a traditional CF models:
% \begin{equation}
%     \frac{a_{n}(j\omega)}{a_{n-1}(j\omega)} = \frac{j(1-k_v H)\omega + k_v}{j\omega + k_v}
%     \label{v_{n}_freq}
% \end{equation}
% As $0 \le k_v H \le 2$ indicates $|1-k_v H| \le 1$, we can ensure that:
% \begin{equation}
%      \left \|\frac{a_{n}(j\omega)}{a_{n-1}(j\omega)} \right\|^2 _2= \frac{[(1-k_v H)\omega]^2 + k_v ^2}{\omega^2 + k_v ^2} \le 1
%     \label{v_{n}_freq}
% \end{equation}
% which satisfies the frequency-domain SS criterion (\cite{naus2010string,Feng2019StringSF}): $\left \|\frac{v_{n}(j\omega)}{v_{n-1}(j\omega)} \right\|_\infty \le 1$, indicating the string-stable property of the linear planner. Note that $\| v(j\omega) \|_\infty = \max _{\omega \in \mathbb{R}} v(j\omega)$, and $\| v(j\omega) \|_2 = \sqrt{\frac{1}{2\pi} \int_{-\infty}^{\infty} \text{Trace} [v(j\omega)^{\dagger}v(j\omega)] d\omega}$
% \end{proof}


% \begin{align}
%     a &= k_v (s-v_{l} H-s_j) + a_l \label{linear-vlead} 
% \end{align}

% Apply the same linear approximation around the equilibrium point, we have:

% \begin{align}
%     \ddot{x_n} &= -k_v H (\dot{x}_{n-1} - \dot{x}_{n-1,eq}) +  k_v (\Delta x_n - \Delta x_{n,eq})  + \ddot{x_{n-1}} - k_v s_j \label{linear-vlead-CF}
% \end{align}



% One can easily find that the linear approximation of a general CF model in \eqref{CF-approx-equil} no longer fits due to the lead vehicle acceleration $\ddot{x_{n-1}}$ introduced here. Consequently, the equivalent condition \eqref{SS-cond-CF} for the SS of a linearized CF model cannot apply.

% To analysis the SS property of \label{linear-vlead-CF}, we first convert it into the expression that involves car-following equilibrium:
% \begin{align}
%     \dot{v} = f(s, v, \Delta v) = f_s s + f_v v + f_{\Delta v} \Delta v
%     \label{acc_eq}
% \end{align}
% where $f_s=k_v$, $f_v=1-k_v H$, $s=x_l-x$, $\Delta v=v_l-v$, and the equilibrium is $(0, v_{eq}, 0)$. Then, apply the perturbation-based method in \cite{wilson2011car}, the SS condition can be obtained as:
% \begin{align}
%     k_v H \ge 0
%     \label{ss-perturb}
% \end{align}
% which is less strict compared to the SS condition derived from frequency-domain method \cite{Feng2019StringSF}: $0\le k_v H \le 2$. Moreover, not all parameters satisfying condition \label{ss-perturb} can imply desired SS (will be shown in the numerical simulations), which validates our argument that the condition in \cite{wilson2011car} might not be feasible in the real-world car-following process.

% \subsection{ Dampening condition in natural driving}


% We can first analyze a simple sinusoidal wave where the lead vehicle is causing a "non-small" perturbation by accelerating first then decelerating to its stable speed. Notice that the lead vehicle's acceleration at the peak of the sinusoidal wave at time $T$ is zero, i.e. $\ddot{x_{n-1}}(T)=0$. To guarantee dampening of the follower, the follower is expected to have a smaller amplitude in its speed profile, and by shifting the response time $\tau$, we expect the acceleration of the follower at time $T+\tau$ to be zero. Assuming the lead vehicle acceleration at time $T+\tau$ remains at zero or is close to zero, we have which means:

% \begin{align}
%     a(T+\tau) = k_v [s(T+\tau)-H \cdot v_l (T+\tau)] + \le 0 \iff s(T+\tau) \le v_l (T+\tau) \cdot H \label{dampening_cond}
% \end{align}

% The dampening condition \eqref{dampening_cond} indicates, for the simplest distance-reaction model, the dampening of the follower vehicle depends on whether the spacing at time $T$ is small enough such that the follower will start to decelerate after $\tau$. \textbf{It is consistent with our finding in the low-level controller paper, because only faster controller can guarantee smaller spacing in the acceleration case, which brings the dampening speed pattern.}


% \textbf{The proof of dampening condition lies in the acceleration to acceleration transfer function}

% When the lead vehicle speed profile experiences continuous waves which can be viewed as a sum of sinusoids with different frequencies.   


% \textbf{It is interesting to derive $\tau$ of a linear ACC model}

% We assume the $\tau$ is a constant, to guarantee the dampening at every cycle, the follower acceleration is expected to be zero at each "crest" and "trough" on the sine waves. Let $i$ denote the index of a crest or trough, then we have:

% \begin{align}
%     a(T_i + \tau) = k_v (s(T_i + \tau)-v_l (T+\tau)) &\le 0 \iff s(T_i+\tau) \le v_l (T_i+\tau) H \nonumber \\
%     \hat{t} \sum_{j=0}^{\floor{T_i+\tau/\hat{t}}} v_{rel}(j \hat{t}) &\le v_l(T_i + \tau) \label{sine-waves}
% \end{align}

% To guarantee dampening in all cycles, the condition \eqref{sine-waves} needs to hold $\forall i$.

% We can also show that, if the linear model dampens at top or valley $i$, it will dampen at next top or valley $i+1$ 
% \begin{proof}
%  \begin{align*}
%     s(T_i + \tau) & \le v_l(T_i + \tau) H ~~~ \text{if it dampens at $i$} \\
%      s(T_{i+1}+\tau) &= s(T_i + \tau) + \hat{t} \sum_{j=\floor{T_i+\tau/\hat{t}}}^{\floor{T_{i+1}+\tau/\hat{t}}} v_{rel}(j \hat{t}) \\
%       &  \le v_l(T_i + \tau)H + \hat{t} \sum_{j=\floor{T_i+\tau/\hat{t}}}^{\floor{T_{i+1}+\tau/\hat{t}}} v_{rel}(j \hat{t}) \\
%       &\le v_l (T_{i}+\tau) H + \Bar{a}_l |_{T_i + \tau} ^{T_{i+1}+\tau} (T_{i+1}-T_i)H\\
%       &\le v_l (T_{i+1}+\tau) H
%  \end{align*}
 
% \end{proof}


% \subsection{Acceleration constraints in factory ACC}
% Now we show how Openpilot computes acceleration bounds for its linear ACC planner:

% \begin{algorithm}
%  \caption{Acceleration constraints in linear ACC at Openpilot, Comma.ai}
%  \begin{algorithmic}[1]
%  \text{}
% \STATE Obtain $a_{min}, a_{max}$ from interpolating a linear acceleration bound model 
% \STATE $a_{max} = a_{max} + interp(v_{ego}, _A_CORR_BY_SPEED_BP, _A_CORR_BY_SPEED_V)  clip(-v_rel / 4., -.5, 1)$\\
% \label{ACC-v_{pid}}
%  \end{algorithmic} 
%  \end{algorithm}
% \FloatBarrier

% \subsection{Differences between SS and dampening}

% Now we show, the expected dampening property of a CF model is not guaranteed by SS. 

% \subsection{Accuracy for a regular linear CF model}
% Now we assume that the desired spacing depends on ego vehicle speed $v$ and the desired acceleration does not require the lead vehicle acceleration. Mathematically, the linear CF model should follow the OVRV model in \eqref{OVRV_model}. 

% From \eqref{SS-cond-linear-model}, one can see if $H$, $k_1$ and $k_2$ are all constant, the SS of the OVRV model should not vary along different speed levels. Based on this, we will study whether this condition can hold  

% \subsection{SS condition for MPC planner}

% To apply the linear approximation of a CF model \eqref{CF-approx-equil} to an MPC controller, one has to compute the derivative \eqref{derivatives} numerically. 

% \subsection{New indexes}
% Notice that the SS indexes we derived here different than what is typically used in control theory. We argue that the indexes here lead some advantages: i) it does not require an equilibrium initial state; ii) it better implies the impact of lead speed change and iii) it 





% The condition in \eqref{SS-cond-CF} is friendly and easy-to-use, which encourages follow-up studies from traffic community \citep{gunter2019model} to design linear CF models that satisfy the condition to achieve SS in simulation. For example, \cite{gunter2019model} adopted the OVRV model in \cite{wilson2011car}:

% \begin{align}
%     \dot{v} = f(s,v,\Delta v) &= k_1 (s-\eta - H v) + k_2 \Delta v \nonumber \\
%     & = -H k_1 \cdot v + k_1\cdot s + k_2 \Delta v  -\eta k_1 \label{OVRV_model}
% \end{align}

% View the OVRV as a general CF model and apply the linear approximation using \eqref{CF-approx} and \eqref{CF-approx-equil}, we can get the acceleration of vehicle $n$ around the equilibrium point:

% \begin{align}
%     \ddot{x_{ego}}-\ddot{x}_{n,eq} & \approx  f_{v} (\dot{x_{ego}}-\dot{x}_{n,eq}) + f_{\Delta x} (\Delta x_{ego}-\Delta x_{n,eq})  + f_{\Delta v} (\Delta \dot{x}_{ego} - \Delta \dot{x}_{n,eq}) \\
%     \ddot{x_{ego}} & \approx f_{v} (\dot{x_{ego}}-\dot{x}_{n,eq}) + f_{\Delta x} (\Delta x_{ego}-\Delta x_{n,eq}) + f_{\Delta v} (\Delta \dot{x}_{ego})\\
%     \dot{v} & \approx -H k_1 \cdot (v-v_{eq}) + k_1\cdot (s-s_{eq}) + k_2 \Delta v 
% \end{align}
% Apparently we have $f_v = -H k_1$, $f_{\Delta x}=k_1$ and $f_{\Delta v}=k_2$. Apply the SS condition in \eqref{SS-cond-CF}, it requires:
% \begin{align}
%     H^2 k_1^2 + 2H k_1 k_2 -2 k_1 \ge 0 \label{SS-cond-linear-model}
% \end{align}

% The above equation \eqref{SS-cond-linear-model} implies the condition for a string stable OVRV model in \eqref{OVRV_model}. 




% \subsubsection{The issue of SS index for linear model}
% We argue that, the SS condition does not account the acceleration bounds, thus the condition is not accurate even for the simplest linear CF model in \eqref{OVRV_model} with $k_2 = 0$.

% \begin{figure}[htbp]
% \centering
% \begin{subfigure}[t]{0.45\linewidth}
%     \includegraphics[width=\linewidth]{linear/accurate_k.png}
%     \caption{linear CF with constant $H=1.7$ and $k_1=0.7$}
% \end{subfigure}%
% \begin{subfigure}[t]{0.45\linewidth}
%     \includegraphics[width=\linewidth]{linear/double_k_SS.png}
%     \caption{linear CF  with constant $H=1.7$ and $k_1=1.4$}
% \end{subfigure}%
%     \caption{Differences of SS between two linear CF models}
%     \label{linear-simulation}
% \end{figure}

% Notice that, theoretically, the above two settings should both be string stable because $k_1$ and $H$ satisfy the condition in \eqref{SS-cond-linear-model}. However, due to the inexplicit acceleration constraints, we found that the left case is string unstable, and doubling $k_1$ can barely guarantee the SS. In reality $k_1=1.4$ is too large and its SS performance might be worse due to the lagging effect caused by the low-level controllers. 

% As stated above, we found that the factory linear ACC system is actually using $v_l$ to plan its target speed and reacts to the distance discrepancy which is also computed from $v_l$. While this sounds like a trivial change, in fact the SS performances has been dramatically improved. To justify its advantage, we show the comparison results as below. The following Fig.\ref{linear-simulation} shows the varied SS from two linear CF models where the only difference is the adoption of ego speed $v$ or lead speed $v_l$. 

% \begin{figure}[htbp]
% \centering
% \begin{subfigure}[t]{0.45\linewidth}
%     \includegraphics[width=\linewidth]{linear/ACC_vEgo.png}
%     \caption{linear CF using ego speed $v$}
% \end{subfigure}%
% \begin{subfigure}[t]{0.45\linewidth}
%     \includegraphics[width=\linewidth]{linear/ACC_vLead.png}
%     \caption{liearn CF model using lead speed $v_l$}
% \end{subfigure}%
%     \caption{Differences of SS between two linear CF models using ego speed or lead speed}
%     \label{linear-simulation}
% \end{figure}
% \FloatBarrier


% \subsubsection{SS index for MPC}

% To apply the SS condition on a non-linear MPC controller, one has to compute the partial derivatives numerically. 




############################
\subsubsection{A time-domain ODE approach}

The transfer function obtained above indicates that the ratio between the output (follower trajectory) and the input (leader) in the s plane. To provide better intuition, we examine the input-output relationship using a time-domain ODE approach by assuming a general perturbation of a sine wave, where the lead speed is as follows: 

\begin{equation}
    v_{lead}(t) = v_{eq} + M \sin(\omega t) \quad \text{for \quad} t \in [0,w]
    \label{lead-speed-t}
\end{equation}
where $M$ and $\omega$ are the amplitude and frequency of the signal respectively.

For the factory linear ACC model:
\begin{align}
    v_{ego}(t+\Delta t) &= v_{lead}(t) + k_v [x_{lead}(t)-x_{ego}(t)-\tau v_{lead}(t)-\delta]\\
    a_{ego} &= a_{lead} (1-k_v \tau) + k_v (v_{lead}-v_{ego})
    \label{factory-ACC-accel-t}
\end{align}

Substitute \eqref{lead-speed-t} into \eqref{factory-ACC-accel-t}, we have:
\begin{align}
      a_{ego}(t) &= k_v (v_{eq} + M \sin(wt)-v_{ego}(t))+(1-k_v \tau) M w \cos(wt) \\
      \dot{v}_{ego}(t) & = k_v v_{eq} + k_v M \sin(wt)+ (1-k_v \tau) Mw \cos(wt) -k_v v_{ego}(t) \label{ODE}
\end{align}

Solving the differential equation in \eqref{ODE}, we can obtain:
\begin{equation}
    v_{ego}(t) = \frac{k_v^2 v_{eq} +e^{-k_v t} k_v^2 M \tau \omega+ v_{eq} \omega^2 -k_v^2 M \tau \omega \cos(t \omega)  + M(k_v^2-k_v \tau \omega^2 +\omega^2)\sin(t \omega)}{k_v^2 + \omega^2}
    \label{solution-ode-factory}
\end{equation}

\textbf{How can we analyze the ODE theoretically? No maximum can be found analytically.}

\textbf{ODE method only captures the dynamics of the follower in CF state.} When the gap is large enough, the follower might 


In this section, we have applied the traditional transfer function to the factory linear ACC model, and also provide an alternative ODE method in the time-domain for further numerical study on the acceleration limits. It is worth noting that both of the methods require a "small" perturbation where the system dynamics (car following state) still hold. In opposite, if the spacing becomes too large, for example, the leader accelerates faster than the acceleration limit of the follower, then the follower is in free flow state where all the above analysis no longer applies. 


% \subsection{SS and dampening of the factory linear ACC}

% \subsubsection{the time domain approach}
% To assist theoretical analysis, we assume the lead vehicle follows simple sine wave as its speed profile. The perturbation from the equilibrium state can be captured by the amplitude $M$ and frequency $w$ of the signal.

% \begin{equation}
%     v_{lead}(t) = v_{eq} + M \sin(wt) \quad \text{for \quad} t \in [0,w]
%     \label{lead-speed-t}
% \end{equation}
% where $M$ is the amplitude of the signal.

% For the factory linear ACC model:
% \begin{align}
%     v_{ego}(t+\Delta t) &= v_{lead}(t) + k_v [x_{lead}(t)-x_{ego}(t)-\tau v_{lead}(t)-\delta]\\
%     a_{ego} &= a_{lead} (1-k_v \tau) + k_v (v_{lead}-v_{ego})
%     \label{factory-ACC-accel-t}
% \end{align}

% \textbf{Can we use Laplace transform to simplify the ODE and solve it?}

\subsection{Impact of the acceleration limits}
% Assume the lead vehicle uses a simple sine wave as its speed perturbation from the equilibrium state.

% \begin{equation}
%     v_{lead}(t) = v_{eq} + M \sin(wt) \quad \text{for \quad} t \in [0,w]
%     \label{lead-speed}
% \end{equation}
% where $M$ is the amplitude of the signal.
% For the factory linear ACC model:
% \begin{align}
%     v_{ego}(t+\Delta t) &= v_{lead}(t) + k_v [x_{lead}(t)-x_{ego}(t)-\tau v_{lead}(t)-\delta]\\
%     a_{ego} &= a_{lead} (1-k_v \tau) + k_v (v_{lead}-v_{ego})
%     \label{factory-ACC-speed}
% \end{align}

Assume the follower ACC-equipped vehicle has a linear acceleration bound:
\begin{equation}
    \Tilde{a}(v_{ego}) = a_{max} \frac{v_{max}-v_{ego}}{v_{max}}
    \label{linear-a-bound}
\end{equation}

Accordingly, the true acceleration becomes a minimum of the system output and the maximum acceleration:
\begin{equation}
    a_{ego} = \min\{k_v (v_{lead}-v_{ego})+(1-k_v \tau)a_{lead},  a_{max} \frac{v_{max}-v_{ego}}{v_{max}}\}
    \label{linar+acceleration}
\end{equation}

The ODE solution in \eqref{ODE} becomes:
\begin{align}
      a_{ego}(t) &= \min\{k_v (v_{eq} + M sin(wt)-v_{ego}(t))+(1-k_v \tau) M w cos(wt),  a_{max} \frac{v_{max}-v_{ego}(t)}{v_{max}}\} \\
      \dot{v}_{ego}(t) & = \min\{k_v v_{eq} + k_v M sin(wt)+ (1-k_v \tau) Mw cos(wt) -k_v v_{ego}(t),  a_{max}-\frac{a_{max}}{v_{max}} v_{ego}(t) \} \label{ODE-constraint}
\end{align}

Unfortunately, the constrained ODE \eqref{ODE-constraint} cannot be solved analytically. We will show numerical results in the following section.

% \begin{equation}
%     v_{ego}(t) =  -\frac{e^{-k_v t}(-e^{k_v t} \pi^2 v_{eq} - k_v^2 M \pi \tau w - e^{k_v t}k_v ^2 v_{eq} w^2 + e^{k_v t}k_v^2 M \pi \tau w \cos[\frac{\pi t}{w}] - e^{k_v t} M \pi^2 \sin[\frac{\pi t}{w}] + e^{k_v t}k_v M \pi^2 \tau \sin[\frac{\pi t}{w}] - e^{k_v t}k_v^2 M w^2 \sin[\frac{\pi t}{w}]  )}{\pi^2 + k_v^2 w^2}
% \end{equation}

% \begin{align}
%     \Gamma &= \frac{\max_{t \in [0,w]}v_{ego}(t)-v_{eq}}{ \max_{t \in [0,w]} v_{lead}(t)-v_{eq}} \\
%     & = \frac{}{M}
% \end{align}



% \section{Background: SS analysis of a linear CF model}\label{background}
% SS has been studied in control theory for more than sixty years. Although the analytical derivation process includes "unfamiliar" techniques to the traffic flow community, the conditions for the SS of a general CF model is quite straightforward. 

% \subsection{Linear approximation of a CF model}
% A general CF model for vehicle $n$ with parameter $\beta_{ego}$ determines its acceleration $\ddot{x_{ego}}$ as a function of its own speed $\dot{x_{ego}}$ , the spacing $\Delta x_{ego} = x_{lead}-x_{ego}$, and the relative speed $\Delta \dot{x_{ego}} = \dot{x_{lead}} - \dot{x_{ego}}$ is from a leading vehicle $lead$.
% Typically, the SS analysis of a CF model first requires to linearize the CF dynamics around the equilibrium state:
% \begin{align}
%     \Ddot{x}_{ego} &= f_{\beta_{n}}(\dot{x_{ego}} , \Delta x_{ego}, \Delta \dot{x_{ego}})  \\
%      &\approx \ddot{x_{n,eq}} + f_{n,v} (\dot{x_{ego}}-\dot{x_{n,eq}}) + f_{n,\Delta x}(\Delta x_{ego} - \Delta x_{n,eq}) + f_{n,\Delta v}(\Delta \dot{x_{ego}}-\Delta \dot{x_{n,eq}})
%      \label{CF-approx}
% \end{align}
% Notice that the partial derivatives are all taken at the equilibrium state, which means:

% \begin{align}
%     f_{n,v} &= \frac{\partial f}{\partial v}|_{v = v_{n,eq}} \nonumber \\
%     f_{n,\Delta x} & = \frac{\partial f}{\partial \Delta x}|_{\Delta x =\Delta x_{n,eq}} \nonumber  \\
%      f_{n,\Delta v} & = \frac{\partial f}{\partial \Delta v}|_{\Delta v = \Delta v_{n,eq}} \label{derivatives}
% \end{align}
% where $v_{n,eq},\Delta x_{n,eq}, \Delta v_{n,eq}$ correspond to the equilibrium speed, spacing and relative speed which can vary at different speed and spacing levels. Of course, at equilibrium $\ddot{x_{ego}}=0$, $v_{n,eq} = const$ and relative speed $\Delta \dot{x}_{n,eq}=0$. Thus the \eqref{CF-approx} can be simplified as:

% \begin{equation}
%       \Ddot{x_{ego}} \approx f_{n,v} (\dot{x_{ego}}-v_{n,eq}) + f_{n,\Delta x}(\Delta x_{ego} - \Delta x_{n,eq}) + f_{n,\Delta v}(\dot{x_{lead}}-\dot{x_{n}})
%      \label{CF-approx-equil}
% \end{equation}

% The accurate approximation of \eqref{CF-approx-equil} requires the speed $\dot{x_{ego}}$ is close to equilibrium speed, and the lead vehicle changes from equilibrium state as well such that the spacing and relative speed only have "small" deviations from the equilibrium state.

% The issue of the linear approximation of a CF model is obvious. The control literature states the above Taylor expansion is designed to study the impact of a "small" enough perturbation that first appeared in \citep{wilson2011car}. However, to the best of our knowledge, the "small" range has never been clarified. 
% \textbf{It means the CF model is only accurate when the lead vehicle deviates from equilibrium state in a very "small" range. On a wave, the CF model only holds near the deviation point. At the peak, the discrepancy might be large.}
% The accuracy of the linear approximation should depend on the linear property of the CF model itself, which also determines how "small" the perturbation can be. One can imagine that, if the CF model is linear and its derivatives do not change too much at different speed or spacing level, the above approximation would have higher accuracy.  


Assuming the follower accelerates at the maximum using \eqref{accel_bound} from $T_0$ to $T^*$, and combining the speed trajectory in \eqref{max_speed_traj}, the dampening condition in \eqref{accel-limits-impact} becomes:
\begin{align}
    \int_{T_0}^{T^*} v_{lead}(t) dt - v_{lead}^1 - \delta & \leq \int_{T_0}^{T^*}  [(v_0-v_c-a_0/\beta)e^{-\beta t} + a_0/\beta + v_c ] \cdot dt \\
    \int_{T_0}^{T^*} v_{lead}(t) dt - v_{lead}^1 - \delta &\leq \frac{(v_0-v_c-a_0/\beta)}{-\beta} \cdot e^{-\beta t}|_{T_0}^{T^*} + (a_0/\beta + v_c) (T^*-T_0) \\
    \int_{T_0}^{T^*} v_{lead}(t) dt - v_{lead}^1 - \delta &\leq \frac{(\beta v_0-\beta v_c-a_0)}{-\beta^2}  (\frac{\beta v_{lead}^1  - \beta v_c- a_0}{\beta v_0-\beta v_c-a_0}-e^{-\beta T_0}) + (a_0/\beta + v_c) (T^*-T_0) \\
    \int_{T_0}^{T^*} v_{lead}(t) dt - v_{lead}^1 - \delta &\leq 
    \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} - (a_0/\beta + v_c) (\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} +T_0) \\
    (T^*-T_0) \bar{v}_{lead} - v_{lead}^1 - \delta &\leq
    \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} - (a_0/\beta + v_c) (\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} +T_0) \\
    (-\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} -T_0) \bar{v}_{lead} - v_{lead}^1 - \delta &\leq
    \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} - (a_0/\beta + v_c) (\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} +T_0) 
\end{align}

It reduces to: 
\begin{align}
     (-\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta}) \bar{v}_{lead} + (a_0/\beta + v_c) (\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} +T_0)-     \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} 
  &\leq v_{lead}^1 + \delta + T_0 \bar{v}_{lead}\\
    (a_0/\beta + v_c-\bar{v}_{lead}) \frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} + (a_0/\beta + v_c) T_0- \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} 
  &\leq v_{lead}^1 + \delta + T_0 \bar{v}_{lead}
\end{align}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{dampening_broken.png}
    \caption{A string stable linear model fails to dampen the large perturbations}
    \label{fig:margional_dampening_factory}
\end{figure}

Analogous to marginal SS, we define "marginal dampening" as the case where the follower's maximum speed change is equal to the maximum lead speed change. The marginal dampening takes places when the equality holds for \eqref{marginal}, which requires the follower happens to reach the equilibrium spacing when its speed just catches up with the leader, i.e. $s(T^*) = \tau v_{lead}^1+\delta$. 

From \eqref{accel-limits-impact}, one can see the acceleration bound can ruin the dampening condition if the follower is not able to close the extra spacing before its speed equals to the leader speed. Similarly, for the deceleration case, the deceleration limit would undermine the dampening condition if the follower cannot brake enough to the equilibrium spacing $\tau v_{lead}^1+\delta$. \textbf{Unfortunately we don't have an explicit expression for the time $T^*$ due to the acceleration constraints. Instead numerical results will be shown in the next section}.



The dampening condition means the maximum follower speed does not exceed $v_{lead}(T_5)$. 

Let $s(t)$ denote the spacing between two vehicles and $T^*$ denote the time when the follower reaches the same speed as the leader, i.e. $v_{ego}(T^*) =v_{lead}(T^*)= v_{lead}^1$. Note that $T^*>T_1$ because the follower speed change is always lagging.

Substitute $v_{ego}(T^*) =v_{lead}(T^*)= v_{lead}^1$ in \eqref{factory-ACC-vlead}, we have the dampening condition as below:
\begin{align}
    v_{ego}(T^* + \Delta t)   & \leq v_{lead}^1  \nonumber \\
   k_v (s(T^*)-\tau v_{lead}(T^*) -\delta) +v_{lead}(T^*)  & \leq v_{lead}^1 \nonumber  \\
    s(T^*) & \leq \tau v_{lead}^1 + \delta \label{marginal} \\
    \int_{T_0}^{T^*} (v_{lead}(t) - v_{ego}(t)) dt & \leq  \tau v_{lead}^1 + \delta  \nonumber \\
    \int_{T_0}^{T^*} v_{lead}(t) dt - v_{lead}^1 - \delta& \leq \int_{T_0}^{T^*} \min \{v_{ego}^{uc}(t), v_{ego}^c(t) \} \cdot dt 
    \label{accel-limits-impact}
\end{align}
where $v_{ego}^{uc}$ and $v_{ego}^c$ denote the unconstrained desired speed from model and the constrained speed due to acceleration limits.


From \eqref{max_speed_traj}, $T^*$ can be solved:
\begin{align}
     T^* = -1/\beta \cdot \ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})  
\end{align}

\begin{align}
     e^{-\beta T^*} = \frac{\beta v_{lead}^1  - \beta v_c- a_0}{\beta v_0-\beta v_c-a_0}  
\end{align}

Assuming the follower accelerates at the maximum using \eqref{accel_bound} from $T_0$ to $T^*$, and combining the speed trajectory in \eqref{max_speed_traj}, the dampening condition in \eqref{accel-limits-impact} becomes:
\begin{align}
    \int_{T_0}^{T^*} v_{lead}(t) dt - v_{lead}^1 - \delta & \leq \int_{T_0}^{T^*}  [(v_0-v_c-a_0/\beta)e^{-\beta t} + a_0/\beta + v_c ] \cdot dt \\
    \int_{T_0}^{T^*} v_{lead}(t) dt - v_{lead}^1 - \delta &\leq \frac{(v_0-v_c-a_0/\beta)}{-\beta} \cdot e^{-\beta t}|_{T_0}^{T^*} + (a_0/\beta + v_c) (T^*-T_0) \\
    \int_{T_0}^{T^*} v_{lead}(t) dt - v_{lead}^1 - \delta &\leq \frac{(\beta v_0-\beta v_c-a_0)}{-\beta^2}  (\frac{\beta v_{lead}^1  - \beta v_c- a_0}{\beta v_0-\beta v_c-a_0}-e^{-\beta T_0}) + (a_0/\beta + v_c) (T^*-T_0) \\
    \int_{T_0}^{T^*} v_{lead}(t) dt - v_{lead}^1 - \delta &\leq 
    \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} - (a_0/\beta + v_c) (\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} +T_0) \\
    (T^*-T_0) \bar{v}_{lead} - v_{lead}^1 - \delta &\leq
    \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} - (a_0/\beta + v_c) (\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} +T_0) \\
    (-\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} -T_0) \bar{v}_{lead} - v_{lead}^1 - \delta &\leq
    \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} - (a_0/\beta + v_c) (\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} +T_0) 
\end{align}

It reduces to: 
\begin{align}
     (-\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta}) \bar{v}_{lead} + (a_0/\beta + v_c) (\frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} +T_0)-     \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} 
  &\leq v_{lead}^1 + \delta + T_0 \bar{v}_{lead}\\
    (a_0/\beta + v_c-\bar{v}_{lead}) \frac{\ln(\frac{v_{lead}^1 - a_0/\beta - v_c}{v_0-v_c-a_0/\beta})}{\beta} + (a_0/\beta + v_c) T_0- \frac{(\beta v_0-\beta v_c-a_0)e^{-\beta T_0} + \beta (v_c-v_{lead}^1)+ a_0 }{\beta^2} 
  &\leq v_{lead}^1 + \delta + T_0 \bar{v}_{lead}
\end{align}






\section{Planner design}
%Solution: anti-windup planner design}

So far we have found that the acceleration bound in ACC design may undermine the SS, especially when the lead vehicle changes speed abruptly. 


To address this issue, here we propose several planner designs to relax the constraint of the acceleration in order to improve the SS.

\subsection{Incorporate integral term}
\textcolor{red}{try to incorporate integral term in planner to combat acceleration limits}

PIF distance controller

faster P distance controller

\begin{align}
    a = k_p e(t) + k_i \int_{0}^{t} e(\tau) d\tau
    \label{integral-CF}
\end{align}

$e$ is the distance error 

design prevent overshooting 

\subsection{Acceleration bound error}
This type of anti-windup design aims at alleviating the deviation between the control input generated from planner and the acceleration bound can be executed by the vehicle.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{accele/anti-windup.png}
    \caption{Factoring the violation of acceleration limit into error}
    \label{fig:anti-windup}
\end{figure}

As shown in the control diagram in \ref{fig:anti-windup}, the original control input $u_p$ generated from the planner will be pass to the vehicle controller to execute the acceleration $u_b$. However, $u_b$ could be clipped by the acceleration bound of the controller, which create an extra error term feedbacked through multiplying a gain $k_b$. Correspondingly, besides the tracking error, the planner now include an additive error term from the acceleration bound:

\begin{equation}
    u_p = k_p e_p + k_v e_v + k_b(u_b-u_p)
    \label{anti_windup input}
\end{equation}

Then $u_p$ is used as $a_{\text{ego}}$ to compute the planner trajectories.

\subsection{Error-dependent control gain tuning}
The control gain tuning in the planner aims at normalizing the tracking error, and then threshold the control input by the acceleration bound. Specifically, the expression of error-dependent control gain is described as:

\begin{gather}
    k_p = \lambda \frac{a_{\text{max}}(1-\text{exp}(-k_1 \|e_p\|))}{\|e_p\|} \\
    \label{anti_windup kp gain}
    k_v = (1-\lambda) \frac{a_{\text{max}}(1-\text{exp}(-k_2 \|e_v\|))}{\|e_v\|} \\
    \label{anti_windup kv gain}
\end{gather}

where the sensitivity coefficient $\lambda$ satisfies $0 \le \lambda \le 1$.

\subsection{String stability barrier function}

The SSBF is applied to regulate the control input to be string stable:

\begin{equation}
    h_{\text{SSBF}}(v_{\text{ego}},v_{\text{lead}}) = \|v_{\text{lead}}\|_2 ^2 - \|v_{\text{ego}}\|_2 ^2 \label{ssbf}
\end{equation}

If \eqref{ssbf} is positive, the string stability is ensured, otherwise string stability is undermined. Thus, we need to devise control input to render $\dot{h}_{\text{SSBF}}(v_{\text{ego}},v_{\text{lead}})>0$ when the states approaching $h_{\text{SSBF}}(v_{\text{ego}},v_{\text{lead}})=0$. Thus, the following SSBF constraint is developed.

\begin{equation}
    \dot{h}_{\text{SSBF}}(v_{\text{ego}},v_{\text{lead}}) = 2 v_{\text{lead}} a_{\text{lead}} - 2 v_{\text{ego}} a_{\text{ego}} > -h_{\text{SSBF}}(v_{\text{ego}},v_{\text{lead}})
    \label{ssbf_dot}
\end{equation}

Then we adopt the quadratic programming (QP) to revise the original control input generated $a_{\text{lead}}^l$ from the linear planner at a minimum level, while subject to the SSBF constraint. The QP is formulated as follows:
\begin{equation}
\begin{aligned}
\min_{u_i} \quad & \frac{1}{2} \|a_{\text{ego}} - a_{\text{lead}}^l\|_2 ^2 \\
\textrm{s.t.} \quad & \dot{h}_{\text{SSBF}}(v_{\text{ego}},v_{\text{lead}}) > -h_{\text{SSBF}}(v_{\text{ego}},v_{\text{lead}})\\
\end{aligned}
\end{equation}

\subsection{Linear acceleration bound}

The linear acceleration model is frequently applied in the traffic flow related research:
\begin{equation}
    a_{\text{ego}} = \beta(v_c-v_{\text{ego}})
    \label{lin_acc}
\end{equation}
where $v_c$ is the desired speed (e.g., the speed of lead vehicle), $\beta$ is the coefficient to adjust acceleration.

Inspired by \eqref{lin_acc}, the acceleration bound can also be constructed as a speed-dependent one:
\begin{equation}
    a_{\text{max}} = \beta(v_c-v_{\text{ego}})
    \label{lin_acc_bound}
\end{equation}
Under the linear acceleration bound \eqref{lin_acc_bound}, the linear planner will become a hybrid switching system:
\begin{equation}
    a_{\text{ego}} = \min \{ \beta(v_c-v_{\text{ego}}), k_p e_p + k_v e_v \}
    \label{switch}
\end{equation}

The SS transfer function for each subsystem can be described as:
\begin{align}
    \Gamma _1 (s) &= \frac{\beta}{s+\beta} \\
    \label{switchTF2}
    \Gamma _2 (s) &= \frac{k_v s + k_p}{s^2 + (k_p h + k_v)s + k_p} \\
    \label{switchTF2}
\end{align}
We can notice both subsystems can be SS, if the parameters are all positive.

In addition to being a constant coefficient, $\beta$ can also be a speed-dependent variable similar to the control gain in \eqref{anti_windup kv gain}:
\begin{equation}
    \beta = \frac{a_{\text{max}}(1-\text{exp}(-\alpha \|v_c-v_{\text{ego}}\|))}{\|v_c-v_{\text{ego}}\|}
    \label{switch}
\end{equation}
where $\alpha$ is a coefficient to adjust the how fast the actual acceleration will reach to $a_{\text{max}}$.
















To show the deterioration of dampening given a string stable model, we start testing both of the linear factory ACC and linear CF model with marginal SS.  

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{dampening_broken.png}
    \caption{A string stable linear model fails to dampen the large perturbations}
    \label{fig:margional_dampening_factory}
\end{figure}

Note that the above perturbation is non-cyclic and simulates a normal acceleration from the driver. The dampening condition still holds when the speed increase is small enough, but deteriorates when the lead speed change grows larger.



\subsection{Resonance frequency and worst-case of string instability}
A string-unstable planner can exhibit a resonance frequency. The oscillation will reach to the highest level if the frequency of the cyclic perturbation matches the resonance frequency of the string-unstable planner.





\subsection{Critically-damping condition}

For the step-function type perturbation, the second-order planner would further need to satisfy the condition of critically-damping to ensure dampening perturbation.

Considering the second-order planner in the form of:
\begin{align}
    a_{\text{ego}} = k_p e_p(t) + k_v e_v(t)
    \label{secondPlanner}
\end{align}
where $e_p(t) = x_{\text{lead}}(t) - x_{\text{ego}}(t) - \tau v_{\text{ego}}(t)$, and $e_v(t) = v_{\text{lead}}(t) - v_{\text{ego}}(t)$. The corresponding SS transfer function will be:
\begin{align}
    \Gamma (s) = \frac{U_{\text{ego}}(s)}{U_{\text{lead}}(s)}  = \frac{k_v s + k_p}{s^2 + (k_p h + k_v)s + k_p}
    \label{SSTF2}
\end{align}
which will be string stable if $k_p>0$ and $k_v>0$.


\textbf{\textit{Comments: The above derivation is the same as the cyclic perturbation case. It might have some problems according to my testing. The transfer function method may only apply to cyclic signals, because essentially they are using Fourier transformation which assumes the cyclic signals. And how do we include the acceleration bound here? }}



The critically-damping condition is directly correlated with the roots of \eqref{SSTF2}: if the roots contains any imaginary part, then the output of \eqref{SSTF2} will be oscillatory and lead to overshoot/undershoot given a step-function type perturbation. The undesired overshoot/undershoot will undermine SS. Correspondingly, the damping ratio of SSTF \eqref{SSTF2} is defined as:
\begin{equation}
    \zeta = \frac{k_p h + k_v}{2 \sqrt{k_p}}
    \label{DampingRatio}
\end{equation}
The case of $\zeta<1$ is denoted as under-damped, where the roots of \eqref{SSTF2} contains imaginary part and will lead to string-unstable response of $U_{\text{ego}}$. The case of $\zeta=1$ is denoted as critically-damped, which is a boundary to separate SS and string-unstable response (it is also a critical boundary to determine if the roots of \eqref{SSTF2} contains imaginary part). The case of $\zeta>1$ is called the over-damped, where SS is guaranteed, but the speed and spacing will converge to desired values in a slower pace compared to the case $\zeta=1$.

Therefore, the SS condition for step-function type perturbation will be:
\begin{equation}
    \zeta \ge 1
    \label{SSCond}
\end{equation}
which is also equivalent to:
\begin{equation}
    (k_p h + k_v)^2 - 4\sqrt{k_p} \ge 0
    \label{SSCond1}
\end{equation}
